EUSO-SPB2 Fluorescence Telescope in-flight performance and preliminary results

The Extreme Universe Space Observatory on a Super Pressure Balloon II (EUSO-SPB2) launched from Wanaka, New Zealand on May 13th 2023. Consisting of two optical telescopes, EUSO-SPB2 aimed to search for very high energy neutrinos (E>PeV) via Cherenkov radiation, and ultra high energy cosmic rays (UHECRs, E>EeV) via ultraviolet fluorescence. Building on the EUSO-Balloon (2014) and EUSO-SPB1 (2017) missions, the Fluorescence Telescope (FT) comprises 108 multi-anode photomultiplier tubes at the focus of a one meter entrance diameter Schmidt telescope. The FT pointed down at the atmosphere below the SPB's altitude of 33 km. The mission duration was planned to reach up to 100 days. Prior to flight, the instrument was extensively tested in the laboratory and in the field. These measurements, combined with simulations led to an expected peak energy sensitivity around 3 EeV. Combined with a three-times-larger field-of-view than previous EUSO balloon missions, this resulted in an expected observation rate of one UHECR shower per ten hours of observation. The FT was expected to perform the first measurement of UHECRs via fluorescence from sub-orbital space, but was unable to, due to a shortened flight. Nonetheless, these observations of EUSO-SPB2 serve as a stepping stone to future satellite-based missions, such as the Probe of Extreme MultiMessenger Astrophysics (POEMMA), with enormous exposure to the highest energy cosmic rays with all sky coverage. In this contribution we will discuss the performance of the FT in flight as well as preliminary results.

==> colors.tex <==
%https://www.mines.edu/webcentral/colors/
\definecolor{MinesDarkBlue}{rgb}{0.1294117647,0.19215686274,0.30196078431}
\definecolor{MinesLightBlue}{rgb}{0.5725490196 ,0.63529411764,0.74117647058}
\definecolor{MinesAccent}{rgb}{0.82352941176,0.2862745098,0.16470588235}

\definecolor{MinesBlue}{rgb}{0.14901960784,0.24705882352,0.41568627451}
\definecolor{MinesPaleBlue}{rgb}{0.80784313725,0.83529411764,0.86666666666}
\definecolor{MinesCoolGray}{rgb}{0.69803921568,0.70588235294,0.70196078431}
\definecolor{MinesMetallic}{rgb}{0.54509803921,0.55294117647,0.55686274509}
